Generalization-Enhanced Code Vulnerability Detection via Multi-Task Instruction Fine-Tuning

Code Pre-trained Models (CodePTMs) based vulnerability detection have achieved promising results over recent years. However, these models struggle to generalize as they typically learn superficial mapping from source code to labels instead of understanding the root causes of code vulnerabilities, resulting in poor performance in real-world scenarios beyond the training instances. To tackle this challenge, we introduce VulLLM, a novel framework that integrates multi-task learning with Large Language Models (LLMs) to effectively mine deep-seated vulnerability features. Specifically, we construct two auxiliary tasks beyond the vulnerability detection task. First, we utilize the vulnerability patches to construct a vulnerability localization task. Second, based on the vulnerability features extracted from patches, we leverage GPT-4 to construct a vulnerability interpretation task. VulLLM innovatively augments vulnerability classification by leveraging generative LLMs to understand complex vulnerability patterns, thus compelling the model to capture the root causes of vulnerabilities rather than overfitting to spurious features of a single task. The experiments conducted on six large datasets demonstrate that VulLLM surpasses seven state-of-the-art models in terms of effectiveness, generalization, and robustness.

==> figures/feature.tex <==
\begin{figure}[t!]
	\centering
    \setlength{\belowcaptionskip}{-10pt}
	\includegraphics[width=1\linewidth]{figures/feature_figure.pdf}
	\centering
	\vspace{-3mm}
	\caption{A example of vulnerability feature extraction. \civi{Can we show the patch in the left figure, and also draw the corresponding PDG?}}
	\label{fig:feature}
\end{figure} 

==> tables/adversarial_table1.tex <==
\begin{table}[htb]
  \centering
  \small
  \renewcommand{\arraystretch}{1.2}
  \setlength\tabcolsep{1.2mm}
  
\begin{tabular}{c|rr|rr|rr}
\toprule
\multirow{2}{*}{Methods}    & \multicolumn{2}{c|}{MHM}     & \multicolumn{2}{c|}{WIR} & \multicolumn{2}{c}{DCI}        \\ 
&\multicolumn{1}{c}{DiV}    & \multicolumn{1}{c|}{ReV}  &\multicolumn{1}{c}{DiV}    & \multicolumn{1}{c|}{ReV} &\multicolumn{1}{c}{DiV}    & \multicolumn{1}{c}{ReV} \\ 
\midrule 
Devign     & & & & & & \\
ReVeal     & & & & & & \\
\midrule 
CodeBERT  &18.10 &9.34  &4.19 &0.41 &35.57 &16.34 \\
GCBERT    &13.33 &9.50  &2.90 &1.12 &28.22 &10.30 \\
UniXcoder &24.97 &20.48 &4.42 &2.18 &37.78 &31.94 \\
\midrule
ReGVD     & & & & & & \\
EPVD      &16.61 &9.77 &4.29 &0.63 &37.08 &16.74 \\
\midrule
VulLLM                 
&\textbf{33.22}   &\textbf{40.06}           &\textbf{16.91}   &\textbf{25.25}  &\textbf{42.32} &\textbf{46.94}   \\ 
\bottomrule

\end{tabular}
\caption{\label{tab:adversarial}The F1 scores under adversarial attacks. For simplicity, GCBERT denotes the GraphCodeBERT model. DCI denotes the Dead Code Insertion attack. Div denotes the DiverseVul dataset, and ReV denotes the ReVeal dataset.}
\vspace{-3mm}
\end{table}

==> tables/eval_results_on_four_datasets.tex <==
\begin{table*}[htb]
  \centering
  \vspace{-2mm}
  \small
  \caption{The evaluation results on the four datasets}
  \renewcommand{\arraystretch}{1.0}
  \setlength\tabcolsep{1mm}
  \label{tab:results_on_four_datasets}
  % \resizebox{0.95\linewidth}{!}{   

\begin{tabular}{c|c|r|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Model}     & \multicolumn{1}{c|}{\multirow{2}{*}{Size}} & \multicolumn{2}{c|}{MixVul}     & \multicolumn{2}{c|}{ReVeal}     & \multicolumn{2}{c|}{Big-Vul}    & \multicolumn{2}{c|}{Juliet}     & \multicolumn{2}{c}{Avg}         \\ \cline{4-13} 
                        &                            & \multicolumn{1}{c|}{}                      & ACC            & F1             & ACC            & F1             & ACC            & F1             & ACC            & F1             & ACC            & F1             \\ \Xhline{1pt}
\multirow{5}{*}{FT}     & CodeBERT                   & 125M                                       & 66.70          & 64.51          & 57.59          & 62.71          & 60.68          & \textbf{64.56} & 51.14          & 67.11          & 59.03          & 64.72          \\
                        & GraphCodeBERT              & 125M                                       & 65.65          & 67.31          & 56.36          & 56.47          & 60.09          & 57.35          & 51.33          & 09.66          & 58.36          & 47.70          \\
                        & UniXcoder                  & 125M                                       & 66.11          & 64.68          & 59.37          & 52.64          & 60.94          & 55.33          & 57.99          & 52.92          & 61.10          & 56.39          \\ \cline{2-13} 
                        & \multirow{2}{*}{CodeLlama} & 7B                                         & 60.62          & 68.08          & 54.19          & 65.48          & \textbf{64.44} & 62.25          & 50.44          & 66.85          & 57.42          & 65.67          \\
                        &                            & 13B                                        & 64.57          & 66.45          & 59.76          & 64.98          & 61.88          & 53.73          & 55.90          & 64.14          & 60.53          & 62.33          \\ \Xhline{1pt}
\multirow{2}{*}{VulLLM} & \multirow{2}{*}{CodeLlama} & 7B                                         & 65.37          & \textbf{69.14} & 59.47          & \textbf{65.95} & 59.49          & 63.98          & 60.95          & 69.66          & 61.32          & \textbf{67.18} \\
                        &                            & 13B                                        & \textbf{68.03} & 68.59          & \textbf{60.01} & 58.47          & 59.57          & 48.64          & \textbf{68.12} & \textbf{75.47} & \textbf{63.93} & 62.79          \\ \Xhline{1pt}
\end{tabular}

  
  % }
  % \begin{tablenotes}
  %   \item $\star$ All results are averaged over the 10 repeated experiments. Metrics-best and Sequence-best denote the models that perform the best among the category of approaches as revealed in the previous research questions, while Metrics-worst and Sequence-worst denote the models that perform the worst.
  % \end{tablenotes}
\end{table*}
